A Geometric Perspective towards Neural Calibration via Sensitivity Decomposition

It is well known that vision classification models suffer from poor calibration in the face of data distribution shifts. In this paper, we take a geometric approach to this problem. We propose Geometric Sensitivity Decomposition (GSD) which decomposes the norm of a sample feature embedding and the angular similarity to a target classifier into an instance-dependent and an instance-independent component. The instance-dependent component captures the sensitive information about changes in the input while the instance-independent component represents the insensitive information serving solely to minimize the loss on the training dataset. Inspired by the decomposition, we analytically derive a simple extension to current softmax-linear models, which learns to disentangle the two components during training. On several common vision models, the disentangled model outperforms other calibration methods on standard calibration metrics in the face of out-of-distribution (OOD) data and corruption with significantly less complexity. Specifically, we surpass the current state of the art by 30.8% relative improvement on corrupted CIFAR100 in Expected Calibration Error. Code available at https://github.com/GT-RIPL/Geometric-Sensitivity-Decomposition.git.

==> figure/decomp_diagram.tex <==
\begin{figure}
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=1.0\textwidth]{figure/decompose_a.png}
         \caption{Decomposition}
         \label{fig:decompose}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=1.0\textwidth]{figure/decompose_b.png}
         \caption{Disentangled Training}
         \label{fig:training}
     \end{subfigure}
        \caption{\textbf{Geometric Sensitivity Decomposition} a) shows the proposed decomposition where $\alpha = \frac{1}{\cos \mathcal{C}_\phi}$ and $\beta = \frac{ \mathcal{C}_x}{\cos \mathcal{C}_\phi} $}
\end{figure}

==> figure/hendryks.tex <==
\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=1.0\textwidth]{figure/hendryks_noisetypes.png}
         \caption{Common Corruptions}
         \label{fig:common_corruptions}
     \end{subfigure}
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=1.0\textwidth]{figure/hendryks_severity.png}
         \caption{5 levels of severity}
         \label{fig:corrupt_levels}
     \end{subfigure}
     \caption{Examples of common corruptions and the 5 levels of severity from \cite{hendrycks2019robustness}.}
\end{figure}

==> table/cifar100_noise.tex <==
\begin{table*}
\centering
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{c|ccc|ccc|ccc|c|c}  
\toprule
& \multicolumn{3}{c}{ECE} & \multicolumn{3}{c}{NLL}& \multicolumn{3}{c}{Brier}& EA-Correl & Accuracy\\
\midrule
Noise-level& 0&3&5 & 0&3&5 & 0&3&5 &all &0\\
\midrule
Ensemble  & \underline{0.024} & \textbf{0.078} & \textbf{0.149}
          & \textbf{0.687} & \textbf{1.969} & \textbf{2.99}
          & \textbf{0.003} & \textbf{0.006} & \textbf{0.008}
          & -0.916 & \textbf{0.816}\\
MCDO & 0.054$\pm$0.002&0.148$\pm$0.006 &0.255$\pm$0.014 
     & 0.941$\pm$0.007&2.236$\pm$0.043 &3.585$\pm$0.119 
     &\textbf{0.003$\pm$0.0}&\textbf{0.006$\pm$0.0} &\underline{0.009$\pm$0.0} 
     &\underline{-0.918$\pm$0.052} &0.766$\pm$0.003\\
\midrule
Vanilla & 0.054$\pm$0.005&0.152$\pm$0.004&\underline{0.237$\pm$0.01}
        & \underline{0.859$\pm$0.006}&2.326$\pm$0.029 &3.434$\pm$0.032 
        & \textbf{0.003$\pm$0.0}&\underline{0.007$\pm$0.0} &\underline{0.009$\pm$0.0}  
        &-0.915$\pm$0.047 & \underline{0.79$\pm$0.002}\\

\midrule
Ours &\textbf{0.023$\pm$0.002} & \underline{0.083$\pm$0.005} & \textbf{0.149$\pm$0.009}
     &0.916$\pm$0.004 & \underline{2.277$\pm$0.013} & \underline{3.199$\pm$0.029}
     &\textbf{0.003$\pm$0.0} &\textbf{0.006$\pm$0.0} &\textbf{0.008$\pm$0.000}
     &\textbf{-0.968$\pm$0.012} &0.78 $\pm$0.003\\
\bottomrule
\end{tabular}}
\caption{Cifar100 Noise}
\label{tab:cifar100_noise}
\end{table*}


==> table/cifar10_noise.tex <==
\begin{table*}
\centering
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{c|ccc|ccc|ccc|c|c}  
\toprule
& \multicolumn{3}{c}{ECE} & \multicolumn{3}{c}{NLL}& \multicolumn{3}{c}{Brier}& EA-Correl & Accuracy\\
\midrule
Noise-level& 0&3&5 & 0&3&5& 0&3&5  &all & 0 \\
\midrule
Ensemble & \textbf{0.006} & \underline{0.076} & \underline{0.184} 
         & \textbf{0.118} & \textbf{0.753} & \underline{1.551}
         & \textbf{0.006} & \textbf{0.03} & \underline{0.057}
         & \underline{-0.966} & \textbf{0.964}\\
MCDO  & 0.015$\pm$0.001&0.102$\pm$0.002 &0.251$\pm$0.008 
      &0.181$\pm$0.006&0.831$\pm$0.013 &1.947$\pm$0.054 
      &0.008$\pm$0.0&0.032$\pm$0.0 &0.065$\pm$0.001 
      &-0.946$\pm$0.033 &0.946$\pm$0.001
\\
\midrule
Vanilla  & 0.026$\pm$0.001&0.153$\pm$0.007 &0.293$\pm$0.016
        & 0.182$\pm$0.003&1.043$\pm$0.046 &2.052$\pm$0.133
        & \underline{0.007$\pm$0.0}&0.038$\pm$0.001 &0.068$\pm$0.002
        &-0.961$\pm$0.046 &\underline{0.955$\pm$0.001}
\\
\midrule
Ours & \underline{0.011$\pm$0.001} & \textbf{0.06$\pm$0.005} & \textbf{0.106$\pm$0.012}
     &\underline{0.166$\pm$0.005} & \underline{0.785$\pm$0.013} & \textbf{1.346$\pm$0.02}
     & \underline{0.007$\pm$0.0} & \underline{0.034$\pm$0.0} & \textbf{0.056$\pm$0.0011}
     & \textbf{-0.975$\pm$0.009} &0.954$\pm$0.002\\
\bottomrule
\end{tabular}}
\caption{Cifar10 Noise}
\label{tab:cifar10_noise}
\end{table*}

==> table/cifar10_rotate.tex <==
\begin{table*}
\centering
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{c|ccccc}  
\toprule
 & ECE & NLL & Brier & EA-Correl & Accuracy\\
\midrule
Ensemble &\textbf{0.302} &\underline{2.397} &\textbf{0.082}&-0.969&\textbf{0.44}\\
MCDO &0.373$\pm$0.001&3.08$\pm$0.025&0.092$\pm$0.0&-0.965$\pm$0.002&0.401$\pm$0.002 \\
\midrule
ResNet18 &0.42$\pm$0.009&2.941$\pm$0.085&0.095$\pm$0.001&-0.968$\pm$0.002& \underline{0.427$\pm$0.006}

\\
% SNGP & \\
\midrule
Ours & \underline{0.323$\pm$0.006} &\textbf{2.211$\pm$0.04} &\underline{0.085$\pm$0.001} &-0.956$\pm$0.006&0.422$\pm0.005$\\
\bottomrule
\end{tabular}}
\caption{CIFAR10 Rotate}
\label{tab:cifar10_rotate}
\end{table*}

==> table/cifar10_svhn_auroc.tex <==
\begin{table*}
\centering
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{c|c|ccc}  
\toprule
& Uncertainty &CIFAR10 vs. SVHN & CIFAR100 vs\\
\midrule
Ensemble & Predictive Entropy\\
MCDO & Predictive Entropy\\
\midrule
CNP& Predictive Entropy\\
ResNet & Softmax Entropy\\
ResNet & Norm\\
DUQ & Kernel Distance\\
SNGP & Predictive Entropy\\
\midrule
Hybrid & Norm\\
Hybrid & Projection\\ 
\bottomrule
\end{tabular}}
\caption{OOD AUROC}
\label{tab:ood}
\end{table*}

==> table/cifar_c.tex <==
\begin{table}[h]
    \begin{subtable}[h]{0.5\textwidth}
        \resizebox{1.0\linewidth}{!}{
        \begin{tabular}{c|cc|cc}  
        \toprule
        \midrule
         Method & \multicolumn{2}{c}{Accuracy} & \multicolumn{2}{c}{ECE} \\
         & Clean & Corrupted & Clean & Corrupted \\
         \midrule
        Vanilla  &\underline{96.0$\pm$0.01} &72.9$\pm$0.01 &0.023$\pm$0.002 &0.153$\pm$0.011 \\
        \midrule
        Ensembles &\textbf{96.6$\pm$0.01} & \textbf{77.9$\pm$0.01} & \textbf{0.010$\pm$0.001} & \underline{0.087$\pm$0.004} \\
        \midrule
        DUQ &94.7$\pm$0.02 &71.6$\pm$0.02 &0.034$\pm$0.002 &0.183$\pm$0.011 \\
        SNGP &95.9$\pm$0.01 &74.6$\pm$0.01 &\underline{0.018$\pm$0.001} &0.090$\pm$0.012 \\ 
        \midrule
        Ours &95.9$\pm$0.01 & \underline{74.9$\pm$0.05} & \underline{0.018$\pm$0.003} & \textbf{0.067$\pm$0.001}\\
            %     Ours &95.9$\pm$0.01 & \underline{74.9$\pm$0.05} & \underline{0.014$\pm$0.001} & \textbf{0.067$\pm$0.001}\\
        \bottomrule
        \end{tabular}
        }
        \caption{\textbf{CIFAR10C}}
        \label{tab:cifar10c}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.5\textwidth}
        \resizebox{1.0\linewidth}{!}{
         \begin{tabular}{c|cc|cc}  
        \toprule
        \midrule
          Method & \multicolumn{2}{c}{Accuracy} & \multicolumn{2}{c}{ECE} \\
         & Clean & Corrupted & Clean & Corrupted \\
         \midrule
        Vanilla &79.8$\pm$0.02 & \underline{50.5$\pm$0.04} &0.085$\pm$0.004 &0.239$\pm$0.020 \\
        \midrule
        Ensembles &\textbf{80.2$\pm$0.01} & \textbf{54.1$\pm$0.04} & \textbf{0.021$\pm$0.004} &0.138$\pm$0.013 \\
        \midrule
        DUQ &78.5$\pm$0.02 &50.4$\pm$0.02 &0.119$\pm$0.001 &0.281$\pm$0.012 \\
        SNGP &\underline{79.9$\pm$0.03} &49.0$\pm$0.02 &\underline{0.025$\pm$0.012} &\underline{0.117$\pm$0.014} \\ 
        \midrule
                % Ours &79.8$\pm$0.03 &49.8 $\pm$ 0.003 & \underline{0.023$\pm$0.003} & \textbf{0.106 $\pm$ 0.008}\\
        Ours &79.8$\pm$0.03 &49.8 $\pm$ 0.003 & 0.027$\pm$0.003 & \textbf{0.081 $\pm$ 0.007}\\
        \bottomrule
        \end{tabular}
            }
        \caption{\textbf{CIFAR100C}}
        \label{tab:cifar100c}
    \end{subtable}
    \caption{Comparison with DUQ and SNGP on CIFAR10/100C with Wide ResNEt 28-10}
\end{table}


